Adversarial Deep Reinforcement Learning based Adaptive Moving Target Defense

Moving target defense (MTD) is a proactive defense approach that aims to thwart attacks by continuously changing the attack surface of a system (e.g., changing host or network configurations), thereby increasing the adversary's uncertainty and attack cost. To maximize the impact of MTD, a defender must strategically choose when and what changes to make, taking into account both the characteristics of its system as well as the adversary's observed activities. Finding an optimal strategy for MTD presents a significant challenge, especially when facing a resourceful and determined adversary who may respond to the defender's actions. In this paper, we propose a multi-agent partially-observable Markov Decision Process model of MTD and formulate a two-player general-sum game between the adversary and the defender. Based on an established model of adaptive MTD, we propose a multi-agent reinforcement learning framework based on the double oracle algorithm to solve the game. In the experiments, we show the effectiveness of our framework in finding optimal policies.

==> figs/eps.tex <==
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}
    	\begin{axis}[
    	font=\small,
    		title=Exploration Fraction,
    		ymin=0, ymax=1.1,
    		xmin=0,	xmax=5.5,
    		width=\linewidth, height=5cm,
            axis x line=middle,
            axis y line=middle,
            ylabel=$\epsilon_\tau$,
            xlabel=Steps in training,
    % 		grid=both,
    %         grid style={line width=.1pt, draw=gray!10},
    %         major grid style={line width=.1pt,draw=gray!10},
    %         minor tick num=1,
    %         enlargelimits={abs=0.5},
            xtick={0, 1, 5},
            xticklabels={0, $\epsilon_p\cdot T\cdot N_e$, $T\cdot N_e$},
            ytick={0, 0.2, 1},
            yticklabels={0, $\epsilon_f$, 1}
    	]
    	\addplot [mark=none, color=red] coordinates {
    		(0, 1)
    		(1, 0.2)
    		(5, 0.2)
    	};
    	
    	\end{axis}
    \end{tikzpicture}
    \caption{Change of exploration  $\epsilon_\tau$ over the training steps.}
    \label{fig:eps}
\end{figure}

==> figs/qnetwork.tex <==
\tikzset{%
  every neuron/.style={
    circle,
    draw,
    minimum size=1cm
  },
  neuron missing/.style={
    draw=none, 
    scale=4,
    text height=0.333cm,
    execute at begin node=\color{black}$\vdots$
  },
}

\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tikzpicture}[x=1.5cm, y=1cm, >=stealth]
    
        \foreach \m/\l [count=\y] in {1,2,3,missing,4}
          \node [every neuron/.try, neuron \m/.try] (input-\m) at (0,2.5-\y) {};
        
        \foreach \m [count=\y] in {1,missing,2}
          \node [every neuron/.try, neuron \m/.try ] (hidden-\m) at (2,2-\y*1.25) {};
        
        \foreach \m [count=\y] in {1,missing,2}
          \node [every neuron/.try, neuron \m/.try ] (output-\m) at (4,1.5-\y) {};
        
        \foreach \l [count=\i] in {1,2,3,n}
          \draw [<-] (input-\i) -- ++(-1,0)
            node [above, midway] {$S'_\l$};
        
        \foreach \l [count=\i] in {1,n}
          \node [above] at (hidden-\i.north) {$H_\l$};
        
        \foreach \l [count=\i] in {1,n}
          \draw [->] (output-\i) -- ++(1,0)
            node [above, midway] {$Q_\l$};
        
        \foreach \i in {1,...,4}
          \foreach \j in {1,...,2}
            \draw [->] (input-\i) -- (hidden-\j);
        
        \foreach \i in {1,...,2}
          \foreach \j in {1,...,2}
            \draw [->] (hidden-\i) -- (output-\j);
        
        \foreach \l [count=\x from 0] in {Input, Hidden, Ouput}
          \node [align=center, above] at (\x*2,2) {\l \\ layer};
    
    \end{tikzpicture}}

    \caption{A $Q$-estimator based on a fully-connected feed-forward artificial neural network. Input $S'$ is the flattened observation state $O^p$. Output is the estimate of $Q$-values for each possible action. An agent selects the action with the highest $Q$-value.}
    \label{fig:qestimator}
\end{figure}

